The Social System Identification Problem

The focus of this paper is modeling what we call a Social Radar, i.e. a method to estimate the relative influence between social agents, by sampling their opinions and as they evolve, after injecting in the network stubborn agents. The stubborn agents opinion is not influenced by the peers they seek to sway, and their opinion bias is the known input to the social network system. The novelty is in the model presented to probe a social network and the solution of the associated regression problem. The model allows to map the observed opinion onto system equations that can be used to infer the social graph and the amount of trust that characterizes the links.

==> macros.tex <==
% new symbols
%\newcommand{\force}{\mbox{$\parallel \! \! \! -$}}
\newcommand{\force}{\mbox{$\Vdash$}}

% Hatted english letters
\newcommand{\ghat}{\mbox{$\bm \hat g$}}
\newcommand{\Nhat}{\mbox{$\bm {\hat N}$}}
\newcommand{\Nlow}{\mbox{${N_{\hbox{\tiny low}}}$}}
\newcommand{\Nhigh}{\mbox{${N_{\hbox{\tiny high}}}$}}
\newcommand{\Nmax}{\mbox{${N_{\hbox{\tiny max}}}$}}
\newcommand{\Iul}{\mbox{${I_{\hbox{\tiny ul}}}$}}
\newcommand{\Idl}{\mbox{${I_{\hbox{\tiny dl}}}$}}


% abbreviations for bold english letters (vectors)
\newcommand{\va}{\mbox{${\bf a}$}}
\newcommand{\vah}{\mbox{${\bf \hat a}$}}
\newcommand{\vat}{\mbox{${\bf \tilde a}$}}
\newcommand{\vb}{\mbox{${\bf b}$}}
\newcommand{\vc}{\mbox{${\bf c}$}}

\newcommand{\vp}{\mbox{${\bf p}$}}
\newcommand{\vd}{\mbox{${\bf d}$}}
\newcommand{\rh}{\mbox{${\hat r}$}}

\newcommand{\vx}{\mbox{${\bf x}$}}
\newcommand{\vxt}{\mbox{${\bf \tilde x}$}}
\newcommand{\vh}{\mbox{${\bf h}$}}
\newcommand{\htld}{\mbox{${\tilde h}$}}
\newcommand{\vhh}{\mbox{${\bf \hat h}$}}
\newcommand{\hhat}{\mbox{${\hat h}$}}
\newcommand{\ve}{\mbox{${\bf e}$}}
\newcommand{\vg}{\mbox{${\bf g}$}}
\newcommand{\vgh}{\mbox{${\bf \hat g}$}}
\newcommand{\vq}{\mbox{${\bf q}$}}
\newcommand{\vt}{\mbox{${\bf t}$}}
\newcommand{\vw}{\mbox{${\bf w}$}}
\newcommand{\vdw}{\mbox{${\bf dw}$}}

\newcommand{\vwh}{\mbox{${\bf \hat w}$}}
\newcommand{\wh}{\mbox{${\hat w}$}}
\newcommand{\vwt}{\mbox{${\bf \tilde w}$}}
\newcommand{\wt}{\mbox{${\tilde w}$}}
\newcommand{\vs}{\mbox{${\bf s}$}}
\newcommand{\vsh}{\mbox{${\bf \hat s}$}}
\newcommand{\vst}{\mbox{${\bf \tilde s}$}}
\newcommand{\vr}{\mbox{${\bf r}$}}
\newcommand{\vv}{\mbox{${\bf v}$}}
\newcommand{\vu}{\mbox{${\bf u}$}}
\newcommand{\vy}{\mbox{${\bf y}$}}
\newcommand{\vz}{\mbox{${\bf z}$}}
\newcommand{\vn}{\mbox{${\bf n}$}}
\newcommand{\vnt}{\mbox{${\bf \tilde n}$}}
\newcommand{\ntld}{\mbox{${\tilde n}$}}
\newcommand{\nhat}{\mbox{${\hat n}$}}
\newcommand{\phat}{\mbox{${\hat p}$}}
\newcommand{\vzero}{\mbox{${\bf 0}$}}
\newcommand{\vone}{\mbox{${\bf 1}$}}

% abbreviations for matrices
\newcommand{\mA}{\hbox{{\bf A}}}
\newcommand{\mAh}{\mbox{${\bf \hat A}$}}
\newcommand{\mAt}{\mbox{$\bf \tilde A$}}
\newcommand{\mB}{\hbox{{\bf B}}}
\newcommand{\mBh}{\mbox{${\bf \hat B}$}}
\newcommand{\mC}{\hbox{{\bf C}}}
\newcommand{\mCh}{\mbox{${\bf \hat C}$}}
\newcommand{\mD}{\hbox{{\bf D}}}
\newcommand{\mDt}{\mbox{$\bf \tilde D$}}
\newcommand{\mE}{\hbox{{\bf E}}}
\newcommand{\mG}{\hbox{{\bf G}}}
\newcommand{\mF}{\hbox{{\bf F}}}
\newcommand{\mH}{\hbox{{\bf H}}}
\newcommand{\mHb}{\mbox{${\bf \bar H}$}}
\newcommand{\mHt}{\mbox{${\bf \tilde H}$}}
\newcommand{\mI}{\hbox{{\bf I}}}
\newcommand{\mIh}{\mbox{${\bf \hat I}$}}
\newcommand{\mN}{\hbox{{\bf N}}}
\newcommand{\mM}{\hbox{{\bf M}}}
\newcommand{\mMh}{\mbox{{$\bf \hat M$}}}
\newcommand{\mP}{\hbox{{\bf P}}}
\newcommand{\mQ}{\hbox{{\bf Q}}}
\newcommand{\mR}{\mbox{{$\bf R$}}}
\newcommand{\mRh}{\mbox{{$\bf \hat R$}}}
\newcommand{\mRt}{\mbox{{$\bf \tilde R$}}}
\newcommand{\mS}{\mbox{{$\bf S$}}}
\newcommand{\mSb}{\mbox{{$\bf \bar S$}}}
\newcommand{\mSh}{\mbox{{$\bf \hat S$}}}
\newcommand{\mSt}{\mbox{{$\bf \tilde S$}}}
\newcommand{\mT}{\mbox{{$\bf T$}}}
\newcommand{\mU}{\mbox{{$\bf U$}}}
\newcommand{\mUh}{\mbox{{$\bf \hat U$}}}
\newcommand{\mV}{\mbox{{$\bf V$}}}
\newcommand{\mVh}{\mbox{{$\bf \hat V$}}}
\newcommand{\mW}{\hbox{{\bf W}}}
\newcommand{\mWh}{\mbox{${\bf \hat W}$}}
\newcommand{\mWt}{\mbox{${\bf \tilde W}$}}
\newcommand{\mX}{\mbox{{$\bf X$}}}
\newcommand{\mY}{\mbox{{$\bf Y$}}}
\newcommand{\mZ}{\mbox{{$\bf Z$}}}



%abbreviations for greek letters

\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\grg}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gre}{\varepsilon}
\newcommand{\gep}{\epsilon}
\newcommand{\gz}{\zeta}
\newcommand{\gzh}{\mbox{$ \hat \zeta$}}
\newcommand{\gh}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gthh}{\mbox{$ \hat \theta$}}
\newcommand{\gi}{iota}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gph}{\phi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gsh}{\hat \sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gf}{\varphi}
\newcommand{\gc}{\chi}
\newcommand{\go}{\omega}

%Uppercase Greek

\newcommand{\gG}{\Gamma}
\newcommand{\gD}{\Delta}
\newcommand{\gTh}{\Theta}
\newcommand{\gL}{\Lambda}
\newcommand{\gX}{\Xi}
\newcommand{\gP}{\Pi}
\newcommand{\gS}{\Sigma}
\newcommand{\gU}{\Upsilon}
\newcommand{\gF}{\Phi}
\newcommand{\gO}{\Omega}

%Uppercase bold Greek

\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\vga}{\mbox{$\bm \alpha$}}
\newcommand{\vgb}{\mbox{$\bm \beta$}}
\newcommand{\vgd}{\mbox{$\bm \delta$}}
\newcommand{\vge}{\mbox{$\bm \epsilon$}}
\newcommand{\vgl}{\mbox{$\bm \lambda$}}
\newcommand{\vgr}{\mbox{$\bm \rho$}}
\newcommand{\vgrh}{\mbox{$\bm \hat \rho$}}
\newcommand{\vgrt}{\mbox{$\bm {\tilde \rho}$}}

\newcommand{\vgt}{\mbox{$\bm \gt$}}
\newcommand{\vgn}{\mbox{$\bm \gn$}}
\newcommand{\vgth}{\mbox{$\bm {\hat \tau}$}}
\newcommand{\vgtt}{\mbox{$\bm {\tilde \tau}$}}
\newcommand{\vpsi}{\mbox{$\bm \psi$}}
\newcommand{\vphi}{\mbox{$\bm \phi$}}
\newcommand{\vxi}{\mbox{$\bm \xi$}}
\newcommand{\vth}{\mbox{$\bm \theta$}}
\newcommand{\vthh}{\mbox{$\bm {\hat \theta}$}}

\newcommand{\mgG}{\mbox{$\bm \Gamma$}}
\newcommand{\mgGh}{\mbox{$\hat {\bm \Gamma}$}}
\newcommand{\mgD}{\mbox{$\bm \Delta$}}
\newcommand{\mgDone}{\mbox{$\bm \Delta^{(1)}$}}
\newcommand{\mgDtwo}{\mbox{$\bm \Delta^{(2)}$}}

\newcommand{\mgU}{\mbox{$\bm \Upsilon$}}
\newcommand{\mgL}{\mbox{$\bm \Lambda$}}
\newcommand{\mPsi}{\mbox{$\bm \Psi$}}
\newcommand{\mgX}{\mbox{$\bm \Xi$}}
\newcommand{\mgS}{\mbox{$\bm \Sigma$}}

%Abbreviatians for blackboard bold
\newcommand{\oA}{{\open A}}
\newcommand{\oC}{{\open C}}
\newcommand{\oF}{{\open F}}
\newcommand{\oN}{{\open N}}
\newcommand{\oP}{{\open P}}
\newcommand{\oQ}{{\open Q}}
\newcommand{\oR}{{\open R}}
\newcommand{\oZ}{{\open Z}}

%Abbreviatians for caligraphic letters

\newcommand{\Nu}{{\cal V}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cX}{{\cal X}}

%\newcommand{\rH}{^{ \raisebox{1pt}{$\rm \scriptscriptstyle H$}}}
\newcommand{\rH}{^{*}}
\newcommand{\rT}{^{ \raisebox{1.2pt}{$\rm \scriptstyle T$}}}
\newcommand{\rF}{_{ \raisebox{-1pt}{$\rm \scriptstyle F$}}}
\newcommand{\rE}{{\rm E}}

% mathematical functions and constants
\newcommand{\dom}{\hbox{dom}}
\newcommand{\rng}{\hbox{rng}}
\newcommand{\Span}{\hbox{span}}
\newcommand{\Ker}{\hbox{Ker}}
\newcommand{\On}{\hbox{On}}
\newcommand{\otp}{\hbox{otp}}
\newcommand{\ZFC}{\hbox{ZFC}}
\def\Re{\ensuremath{\hbox{Re}}}
\def\Im{\ensuremath{\hbox{Im}}}
\newcommand{\SNR}{\ensuremath{\hbox{SNR}}}
\newcommand{\SINR}{\ensuremath{\hbox{SINR}}}
\newcommand{\CRB}{\ensuremath{\hbox{CRB}}}
\newcommand{\diag}{\ensuremath{\hbox{diag}}}
\newcommand{\trace}{\ensuremath{\hbox{tr}}}


% more complex mathematical entities
\newcommand{\dlot}{\mbox{$\delta^1_3$}}
\newcommand{\Dlot}{\mbox{$\Delta^1_3$}}
\newcommand{\Dlof}{\mbox{$\Delta^1_4$}}
\newcommand{\dlof}{\mbox{$\delta^1_4$}}
\newcommand{\bP}{\mbox{$\bf{P}$}}
\newcommand{\Pot}{\mbox{$\Pi^1_2$}}
\newcommand{\Sot}{\mbox{$\Sigma^1_2$}}
\newcommand{\gDot}{\mbox{$\gD^1_2$}}

\newcommand{\Potr}{\mbox{$\Pi^1_3$}}
\newcommand{\Sotr}{\mbox{$\Sigma^1_3$}}
\newcommand{\gDotr}{\mbox{$\gD^1_3$}}

\newcommand{\Pofr}{\mbox{$\Pi^1_4$}}
\newcommand{\Sofr}{\mbox{$\Sigma^1_4$}}
\newcommand{\Dofr}{\mbox{$\gD^1_4$}}


\newcommand{\Sa}{\mbox{$S_{\ga}$}}
\newcommand{\Qk}{\mbox{$Q_{\gk}$}}
\newcommand{\Ca}{\mbox{$C_{\ga}$}}

\newcommand{\gkp}{\mbox{$\gk^+$}}
\newcommand{\aron}{ Aronszajn }

\newcommand{\sqkp}{\mbox{$\Box_{\gk}$}}
\newcommand{\dkp}{\mbox{$\Diamond_{\gk^{+}}$}}
\newcommand{\sqsqnce}
{\mbox{\\ $\ < \Ca \mid \ga < \gkp \ \ \wedge \ \ \lim \ga >$ \ \ }}
\newcommand{\dsqnce}{\mbox{$<S_{\ga} \mid \ga < \gkp >$}}


% mathematical environments
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{principle}[theorem]{Principle}
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{claim}{Claim}[section]

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]
%\theoremstyle{remark}
\newtheorem{question}{Question}[section]
\newtheorem{coro}{Corollary}[section]

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{array}}
\newcommand{\ena}{\end{array}}
%\newcommand{\bds}{\begin {description}}
%\newcommand{\eds}{\end {description}}
\newcommand{\bds}{\begin {itemize}}
\newcommand{\eds}{\end {itemize}}
\newcommand{\bdf}{\begin{definition}}
\newcommand{\blm}{\begin{lemma}}
\newcommand{\edf}{\end{definition}}
\newcommand{\elm}{\end{lemma}}
\newcommand{\bthm}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\bprp}{\begin{prop}}
\newcommand{\eprp}{\end{prop}}
\newcommand{\bcl}{\begin{claim}}
\newcommand{\ecl}{\end{claim}}
\newcommand{\bcr}{\begin{coro}}
\newcommand{\ecr}{\end{coro}}
\newcommand{\bquest}{\begin{question}}
\newcommand{\equest}{\end{question}}

%Abbreviatians for other symbols
\newcommand{\rarrow}{{\rightarrow}}
\newcommand{\Rarrow}{{\Rightarrow}}
\newcommand{\larrow}{{\leftarrow}}
\newcommand{\Larrow}{{\Leftarrow}}
\newcommand{\restrict}{{\upharpoonright}}
\newcommand{\nin}{{\not \in}}





%\newcommand{\ha}{\mbox{$\hat{\b{a}}$}}
%\newcommand{\tba}{\mbox{$\tilde{\b{a}}$}}
%\newcommand{\yh}{\mbox{${\hat y}$}}
%\newcommand{\vth}{\mbox{${\boldsymbol {\theta}}$}}
%\newcommand{\ups}{\mbox{${\Upsilon}$}}
%\newcommand{\vthh}{\mbox{${\boldsymbol {\hat \theta}}$}}
%\newcommand{\vtht}{\mbox{${\boldsymbol {\tilde \theta}}$}}
%\newcommand{\veps}{\mbox{${\underline \epsilon}$}}
%\newcommand{\vrho}{\mbox{${\boldsymbol {\rho}}$}}
%\newcommand{\vrhoh}{\mbox{${\boldsymbol {\hat \rho}}$}}
%\newcommand{\vrhot}{\mbox{${\boldsymbol {\tilde \rho}}$}}

%\newcommand{\vy}{\mbox{${\bf y}$}}
%\newcommand{\vyh}{\mbox{${\bf \check y}$}}
%\newcommand{\vyht}{\mbox{${\bf \hat y}$}}
%\newcommand{\vnh}{\mbox{${\bf \check n}$}}
%\newcommand{\omn}{\mbox{${\om_{_N}}$}}
%\newcommand{\pikon}{\mbox{${\frac{2\pi k}{N}}$}}



% Abrreviations
\newcommand{\ie}{\hbox{i.e.}}
\newcommand{\eg}{\hbox{e.g.}}
\newcommand{\Pnx}{\mbox{$P_{\hbox{next}}$}}
\newcommand{\Knx}{\mbox{$K_{\hbox{next}}$}}

